ImageBind-LLM: Multi-modality Instruction Tuning

We present ImageBind-LLM, a multi-modality instruction tuning method of large language models (LLMs) via ImageBind. Existing works mainly focus on language and image instruction tuning, different from which, our ImageBind-LLM can respond to multi-modality conditions, including audio, 3D point clouds, video, and their embedding-space arithmetic by only image-text alignment training. During training, we adopt a learnable bind network to align the embedding space between LLaMA and ImageBind's image encoder. Then, the image features transformed by the bind network are added to word tokens of all layers in LLaMA, which progressively injects visual instructions via an attention-free and zero-initialized gating mechanism. Aided by the joint embedding of ImageBind, the simple image-text training enables our model to exhibit superior multi-modality instruction-following capabilities. During inference, the multi-modality inputs are fed into the corresponding ImageBind encoders, and processed by a proposed visual cache model for further cross-modal embedding enhancement. The training-free cache model retrieves from three million image features extracted by ImageBind, which effectively mitigates the training-inference modality discrepancy. Notably, with our approach, ImageBind-LLM can respond to instructions of diverse modalities and demonstrate significant language generation quality. Code is released at https://github.com/OpenGVLab/LLaMA-Adapter.

==> tabs/application_2.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
\begin{figure*}[tbhp]
    \centering
    \footnotesize
    \resizebox{\textwidth}{!}{%
\begin{tabular}{ll}
\textbf{\textit{\textcolor[HTML]{2090ff}{Speech-to-Text}}}\\
\multirow{2}{*}{
\includegraphics[width=0.17\columnwidth]{figs/instruction_examples/lover.png}
} & \begin{minipage}[t]{\columnwidth}
\textbf{Instruction:} What does this song convey?\\
\textbf{w/o expert:} The audio conveys a message that encourages viewers to "believe in the power of love."\\
\textbf{w/ Speech-to-text expert:} (\textbf{recognized text}: And ah, take me out, and take me home forever and ever. You're my my my my Lover.) The audio conveys a powerful and emotional message, possibly expressing a woman's desire to be with her lover forever. The lyrics suggest a strong, long-lasting bond between the two, and the woman's willingness to commit to this relationship. The song is likely to evoke feelings of love, passion, and devotion, as it is a romantic ballad.
\end{minipage} \\
\\
\textbf{\textit{\textcolor[HTML]{800080}{Video Detection}}}\\
\multirow{2}{*}{
\includegraphics[width=0.17\columnwidth]{figs/instruction_examples/cat_play.png}
} & \begin{minipage}[t]{\columnwidth}
\textbf{Instruction:} What is this cat doing?\\
\textbf{w/o expert:} The cat is standing on a table and watching the two fish swimming in a bowl.\\
\textbf{w/ Video Object Detection expert:} (\textbf{detected classes}: cat, small fish, shrimp, water basin, floor) The cat is standing on the floor next to a water basin, and it appears to be observing or possibly playing with a small fish or shrimp that is swimming in the water.
\end{minipage} \\
\\
\end{tabular}%
}
\caption{\textbf{Advanced Examples by Integrating ImageBind-LLM with Modality Experts}.}
\label{tab:domain_expert}
\end{figure*}

==> tabs/instruction_tuning_examples.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
\begin{figure*}[tbhp]
    \centering
    
    \resizebox{\textwidth}{!}{%
    \footnotesize
\begin{tabular}{ll}
\textbf{\textit{\textcolor[HTML]{004ccd}{Image}}}\\
\multirow{2}{*}{
\includegraphics[width=0.17\columnwidth]{figs/instruction_examples/zelda.png}
} & \begin{minipage}[t]{\columnwidth}
\textbf{Instruction:} Tell me about this game. \end{minipage}\\
& \begin{minipage}[t]{\columnwidth}\textbf{Answer:} The game is called "The Legend of Zelda: Breath of the Wild," which is a popular action-adventure game developed by Nintendo for the Nintendo Switch and the Wii U console. The game is set in the fictional kingdom of Hyrule and follows the story of Link, a young boy who embarks on a quest to save the kingdom and rescue Princess Zelda. The game features open-world exploration, puzzle-solving, and various combat mechanics, making it a highly engaging and immersive experience for players.\end{minipage} \\
\\
% \multirow{2}{*}{
% \includegraphics[width=0.17\columnwidth]{figs/instruction_examples/girl_paint.png}
% } & \begin{minipage}[t]{\columnwidth}
% \textbf{Instruction:} Introduce the painter of this image. \end{minipage}\\
% & \begin{minipage}[t]{\columnwidth}\textbf{Answer:} The painter of this image is Johannes Vermeer, a Dutch painter who was active in the Dutch Golden Age during the 17th century. He is known for his realistic and detailed paintings, often featuring women in domestic settings.\end{minipage} \\
% \\
\multirow{2}{*}{
\includegraphics[width=0.17\columnwidth]{figs/instruction_examples/shanghai.jpg}
} & \begin{minipage}[t]{\columnwidth}
\textbf{Instruction:} What city was this picture taken in and why?\end{minipage}\\
& \begin{minipage}[t]{\columnwidth}\textbf{Answer:} The picture was taken in Shanghai, China. The presence of the tall buildings, the river, and the skyline suggest that the image was captured in a large city with a prominent urban landscape. Shanghai is known for its modern architecture, such as the Oriental Pearl Tower, and its proximity to the Huangpu River, which is a popular tourist attraction. The city's skyline, with its tall buildings and the river, creates a visually appealing and iconic backdrop for the image.\end{minipage} \\
\\
\textbf{\textit{\textcolor[HTML]{2090ff}{Audio}}}\\
\multirow{2}{*}{
\includegraphics[width=0.17\columnwidth]{figs/instruction_examples/bear_bar.png}
} & \begin{minipage}[t]{\columnwidth}
\textbf{Instruction:} How do you feel when you hear this music?\end{minipage}\\
& \begin{minipage}[t]{\columnwidth}\textbf{Answer:} When I hear this music, I feel a sense of adventure and excitement. The combination of the electronic beats, the space-themed imagery, and the red and black color scheme create a thrilling atmosphere that invites listeners to explore new worlds and embark on a journey of discovery. The music may also evoke feelings of freedom and independence, as it may be associated with outer space or other far-off destinations.\end{minipage} \\
\\
\multirow{2}{*}{
\includegraphics[width=0.17\columnwidth]{figs/instruction_examples/sea_wave.png}
} & \begin{minipage}[t]{\columnwidth}
\textbf{Instruction:} Write a poem based on this audio.\end{minipage}\\
& \begin{minipage}[t]{\columnwidth}\textbf{Answer:} Amidst the crashing waves, a lone bird flies;
Soaring high above the ocean's blue sky;
The waves crashing, the winds blowing;
A symphony of nature, a sight to see.\end{minipage} \\
\\
\textbf{\textit{\textcolor[HTML]{800080}{Video}}}\\
\multirow{2}{*}{
\includegraphics[width=0.17\columnwidth]{figs/instruction_examples/your_name.png}
} & \begin{minipage}[t]{\columnwidth}
\textbf{Instruction:} Introduce me this movie.\end{minipage}\\
& \begin{minipage}[t]{\columnwidth}\textbf{Answer:} The movie is titled "Your Name" and is a Japanese animated film released in 2016. It is a heartwarming and emotional story about two teenagers who discover a connection between their lives, and their journey to find the truth behind their shared experience. The film has received widespread critical acclaim and has been a commercial success, winning numerous awards and accolades, including the Academy Award for Best Animated Feature Film. The movie is known for its beautiful animation, captivating storytelling, and thought-provoking themes.\end{minipage} \\
\\
\multirow{2}{*}{
\includegraphics[width=0.17\columnwidth]{figs/instruction_examples/jump.png}
} & \begin{minipage}[t]{\columnwidth}
\textbf{Instruction:} Do you find this sport exciting? Describe this video.\end{minipage}\\
& \begin{minipage}[t]{\columnwidth}\textbf{Answer:} Yes, this sport is exciting, as it showcases the thrilling experience of skydiving while also providing a unique perspective of the landscape below. The video captures the skydivers in mid-air, performing tricks and enjoying the adrenaline rush of the sport. The image of the parachutist flying through the sky with the landscape below is visually stunning and captures the essence of the freedom and adventure associated with skydiving.\end{minipage} \\
\\
\textbf{\textit{\textcolor[HTML]{ffc000}{Point Cloud}}}\\
\multirow{2}{*}{
\includegraphics[width=0.17\columnwidth]{figs/instruction_examples/piano.jpg}
} & \begin{minipage}[t]{\columnwidth}
\textbf{Instruction:} Describe the 3D object in detail.\end{minipage}\\
& \begin{minipage}[t]{\columnwidth}\textbf{Answer:} The 3D object is a grand piano, which is a musical instrument with a keyboard and a set of strings. The piano has a piano keyboard, which consists of white and black keys arranged in a grid-like pattern. The keys are connected to hammers that strike the strings, creating the sound of the piano. The piano in the image is a small, two-tiered model, with a brown and white color scheme. The piano is sitting on top of a bench, which is a standard accompaniment for a piano. The bench has a supportive design that allows the player to sit comfortably while playing the instrument.\end{minipage} \\
\\
\multirow{2}{*}{
\includegraphics[width=0.17\columnwidth]{figs/instruction_examples/flower_bottle.jpg}
} & \begin{minipage}[t]{\columnwidth}
\textbf{Instruction:} Describe the 3D object in detail.\end{minipage}\\
& \begin{minipage}[t]{\columnwidth}\textbf{Answer:} The 3D object is a flower pot with a plant inside it. The plant is a small, green, and leafy plant, which is growing out of the pot. The pot is made of clay and has a brown color. The plant is positioned towards the front of the pot, with its leaves spreading outwards. The pot is placed on a table, and the close-up view of the plant and pot showcases the details of the plant and the pot's design.\end{minipage} \\
\\

\end{tabular}%
}
\caption{\textbf{Multi-modal Instruction Examples with ImageBind-LLM}.}
\label{tab:caption_demo}
\end{figure*}

==> tabs/mixture_of_modalities.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
\begin{figure*}[tbhp]
    \centering
    \footnotesize
    \resizebox{\textwidth}{!}{%
\begin{tabular}{ll}
\textbf{\textit{\textcolor[HTML]{004ccd}{Image}+\textcolor[HTML]{2090ff}{Audio}}}\\
\multirow{2}{*}{
\includegraphics[width=0.17\columnwidth]{figs/instruction_examples/image_audio_1.png}
} & \begin{minipage}[t]{\columnwidth}
\textbf{Instruction:} Guess the girl's mood based on the background music and explain the reason. \end{minipage}\\
& \begin{minipage}[t]{\columnwidth}\textbf{Answer:} The girl in the image appears to be in a contemplative or melancholic mood, as the background music is a sad piano melody. This choice of music suggests that the scene is intended to evoke a sense of introspection, solitude, or longing. The combination of the girl's attire, the lone tree, and the melancholic music creates a mood of introspection and contemplation. The use of such music can help to enhance the emotional impact of the scene and provide a deeper understanding of the character's thoughts and feelings.\end{minipage} \\
\\
\multirow{2}{*}{
\includegraphics[width=0.17\columnwidth]{figs/instruction_examples/image_audio_2.png}
} & \begin{minipage}[t]{\columnwidth}
\textbf{Instruction:} Describe the scene based on the input picture and audio.\end{minipage}\\
& \begin{minipage}[t]{\columnwidth}\textbf{Answer:} The scene depicted in the image is a busy city street filled with traffic. There are numerous cars, trucks, and buses driving down the street, creating a bustling atmosphere. The street is crowded with vehicles, and the traffic appears to be moving slowly. The audio accompanying the image suggests that the traffic is quite congested, with honking and other noises typical of a busy city street. The image captures the essence of urban life, showcasing the hustle and bustle of daily city life.\end{minipage} \\
\\
\textbf{\textit{\textcolor[HTML]{004ccd}{Image}+\textcolor[HTML]{ffc000}{PC}}}\\
\multirow{2}{*}{
\includegraphics[width=0.17\columnwidth]{figs/instruction_examples/image_point_1.png}
} & \begin{minipage}[t]{\columnwidth}
\textbf{Instruction:} Describe this scene. \end{minipage}\\
& \begin{minipage}[t]{\columnwidth}\textbf{Answer:} The image features a blue car driving down a tree-lined road, surrounded by a lush green forest. The car is in the middle of the road, and it appears to be a compact or small vehicle. There are several trees on both sides of the road, creating a serene and peaceful atmosphere. The car is moving along the road, possibly enjoying the scenic beauty of the forest. \\ \end{minipage} \\
\\ \\
\textbf{\textit{\textcolor[HTML]{800080}{Video}+\textcolor[HTML]{2090ff}{Audio}}}\\
\multirow{2}{*}{
\includegraphics[width=0.17\columnwidth]{figs/instruction_examples/video_audio_1.png}
} & \begin{minipage}[t]{\columnwidth}
\textbf{Instruction:} What is the man doing in this video? What do people think of him based on the audio?\end{minipage}\\
& \begin{minipage}[t]{\columnwidth}\textbf{Answer:} The man is standing at a podium, giving a speech or presentation. People in the audience are listening to him attentively, and they are clapping and showing their appreciation for his words.\end{minipage} \\
\\ \\ \\ 


\end{tabular}%
}
\caption{\textbf{Mixture of Modalities with ImageBind-LLM}.}
\label{tab:mix_modality}
\end{figure*}
